A Randomized Algorithm for Sparse PCA based on the Basic SDP Relaxation

Sparse Principal Component Analysis (SPCA) is a fundamental technique for dimensionality reduction, and is NP-hard. In this paper, we introduce a randomized approximation algorithm for SPCA, which is based on the basic SDP relaxation. Our algorithm takes an (approximate) SDP solution, constructs one deterministic sparse solution and several randomized solutions, and outputs the best among them. Our algorithm has an approximation ratio of at most the sparsity constant with high probability, if called enough times. Under a technical assumption, which is consistently satisfied in our numerical tests, the average approximation ratio is also bounded by $\mathcal{O}(\log{d})$, where $d$ is the number of features. We show that this technical assumption is satisfied if the SDP solution is low-rank, or has exponentially decaying eigenvalues. We then present two classes of instances for which this technical assumption holds. We also demonstrate that in a covariance model, which generalizes the spiked Wishart model, the deterministic solution in our algorithm achieves a near-optimal approximation ratio. We demonstrate the efficacy of our algorithm through numerical tests on real-world datasets.

==> sections/comparison.tex <==
\section{Comparison with other polynomial-time algorithms}
	\label{app:comparison}
    In this section, we investigate how our proposed algorithm, \cref{alg:multi_ra}, compares with other known polynomial-time approximation algorithms for~\ref{prob SPCA}. 
    
    We start by giving a time complexity bound of \cref{alg:multi_ra}. 
    We note that solving \eqref{prob SDP SPCA} via an interior point method requires a runtime of $\mathcal{O}(\sqrt{d}d^{2\omega}\textup{Poly}(\log{d}))$, where $d^{\omega}$ represents the time complexity for matrix multiplication. 
    This can be impractical for large-scale instances. 
    However, as discussed in \cref{sec:numerical tests spca}, by leveraging the special structure of \ref{prob SPCA}, it is possible to approximately solve \eqref{prob SDP SPCA} using CGAL within a time complexity of $\mathcal{O}(m \cdot d^2\log{d})$ approximately, where $m$ is the number of CGAL iterations. 
    We provide an introduction to CGAL in \cref{app:extra tests}.
    Furthermore, we denote $N$ as the number of iterations in \cref{alg:multi_ra}. The time complexity for \cref{alg:multi_ra} is thus at most $\mathcal{O}(d\log{d} + N(d + k^2\log{k}))$. 
    
    The results are summarized in \cref{table:comparison}, with the column "Type" indicating the type of approximation bound (multiplicative (M) or additive (A)).
    Note that, as discussed in \cref{sec:rank_one}, we use the stronger results developed in \cite{dey2017sparse,dey2022using} when Assumption~\ref{ass:rank-one} is satisfied.
    In \cite{papailiopoulos2013sparse}, the authors proposed an approximation algorithm that utilizes a rank-$q$ approximation of the input matrix $A$, demonstrating that the algorithm's approximation ratio is influenced by the $q$-th largest eigenvalue $\lambda_q$ of $A$.
    Hence, in the table, we use the integer $q$ to denote the degree of low-rank approximation is used.
    We also note that when characterizing the approximation guarantee of \cref{alg:multi_ra}, we use the notation from \cref{thm:spca rand alg}, specifically $\sqrt{W^*}=(u_1, u_2, \dots, u_d)$.


    \begin{table}[htb]
    \caption{Comparison of Runtime Complexity and Approximation Bound}
    \label{table:comparison}
    \centering
    \begin{tabular}{lccc}
        \toprule
        methods & time complexity & approximation bound & type\\
        \midrule
        Low-rank~\cite{papailiopoulos2013sparse} & $\mathcal{O}(d^{q+1}\log{d})$ & $1 / \left(1- \lambda_{q + 1} \cdot \min\left\{\frac{d}{k\lambda_1}, \frac{1}{\max_{i \in [d]} A_{ii}} \right\} \right)$ & M\\
        Truncation~\cite{chan2016approximability} & $\mathcal{O}(d^3)$ & $\min\{\sqrt{k}, d^{1/3}\}$ & M\\
        Bipartite~\cite{asteris2015sparse} & $\mathcal{O}(d^{\textup{Poly}(1/\epsilon)})$ & $\epsilon$ & A\\
        Greedy~\cite{li2020exact} & $\mathcal{O}(d^3)$ & $k$ & M \\
        Local Search~\cite{li2020exact} & $\mathcal{O}(d^4k)$ & $k$ & M\\
        \cref{alg:multi_ra} & \makecell{$\mathcal{O}(m \cdot d^2 \log{d}$ \\ $+ N\cdot(d + k^2 \log{k}))$} & \makecell{$\mathcal{O}\left(\frac{(\sum_{i = 1}^d \|u_i\|)^2}{k} \log{d}\right)$ in general, \\ constant under Assumption~\ref{ass:rank-one}, \\ and near one in \cref{model:adversarial}} & M\\
        \bottomrule
    \end{tabular}
    \end{table}

    It can be observed that the greedy method and the local search method proposed by \cite{li2020exact} are outperformed by the truncation method from \cite{chan2016approximability}, as they share the same time complexity but the truncation method offers a superior approximation bound. 
    Additionally, the bipartite method proposed by \cite{asteris2015sparse} primarily serves theoretical interests, and its practical implementation remains uncertain.

    Direct comparisons among other methods are challenging. 
    For instance, our \cref{alg:multi_ra} achieves a $\mathcal{O}(\log{d})$-approximation ratio under the technical assumption~\eqref{eqn:spca tech cond}, representing, to the best of our knowledge, the first logarithmic bound of this type for \ref{prob SPCA}. This guarantee is driven by the randomized candidates generated from $W^*$.
    This makes it particularly powerful and more effective than the truncation and greedy methods when $k$ is large (e.g., $k\ge \log^2{d}$). 
    However, when $k$ is small, it becomes less advantageous. 
    Moreover, when \eqref{eqn:spca tech cond} does not hold, the approximation bound of this randomized component could degrade to $\mathcal{O}(d\log{d}/k)$, making it less competitive unless $k \approx d$.
    
    Due to the complexity of these scenarios, in the remainder of the section, we focus on elucidating the advantages of each method under varying conditions rather than directly comparing their time complexity and approximation bounds.    
    We observe that when the input matrix $A$, with eigenvalues $\lambda_1 \ge \lambda_2 \ge \dots \ge \lambda_d$, exhibits a sharp decrease (e.g., exponential decrease, $\lambda_{i+1} / \lambda_{i} \le c < 1$), the low-rank method is particularly suitable as its approximation bound rapidly approaches one with increasing $q$. However, this method may not be computationally efficient for large $d$ and $q$. 
    In scenarios where \ref{prob SDP SPCA} admits a sparse solution, or when the input matrix satisfies Assumption~\ref{ass:rank-one}, or when a specific hidden sparse structure is identified in the data (e.g., the spiked covariance model or \cref{model:adversarial}), the deterministic candidate in \cref{alg:multi_ra} proves highly beneficial. 
    When these structures also imply \eqref{eqn:spca tech cond}, the randomized component still gives the overall algorithm a worst-case $\mathcal{O}(\log{d})$ approximation bound. In \cref{model:adversarial}, the deterministic candidate is even near-optimal, as discussed in \cref{thm:randomized_alg_in_stat_model}. 
    Moreover, our empirical studies indicate considerable efficiency, with feasible settings where $m = 100$ and $N$ can be as low as 100, as reported in \cref{sec:numerical tests spca} and \cref{app:extra tests}. 
    Lastly, when no prior information is available, the truncation and greedy methods are great options, although they may encounter scalability issues for very large $d$.

==> sections/extraempirical.tex <==
\section{Detailed numerical tests}
	\label[appendix]{app:extra tests}
    In this section, we present details of our numerical tests that are not specified in \cref{sec:numerical tests spca}.
 
	\paragraph{Introduction to CGAL.}
    CGAL~\cite{yurtsever2019conditional} is an iterative algorithm that can be used to (approximately) solve the following optimization problem: 
    {\setlength{\abovedisplayskip}{0pt}
  \setlength{\belowdisplayskip}{0pt}%
	\begin{align*}
		f(x^*) := \min  \ f(x) \quad
		\text{s.t. }  x\in \mathcal{X}, \ C x \in \mathcal{K},
	\end{align*}
    }
	where $f$ is a convex and $L$-smooth function, $C$ is a linear mapping, $\mathcal{X}$ is a convex compact set and $\mathcal{K}$ is a convex set. 
	In the $m$-th iteration, CGAL is guaranteed to find a vector $x_m$ such that $|f(x_m) - f(x^*)| \le \mo\left(m^{-1/2}\right)$ and $\text{dist}(C x_m, \mathcal{K}) \le \mo\left(m^{-1/2}\right)$.
	In the tests, number of iterations in CGAL is set to $100$ and $\lambda_0$ is set to $1$, and we initialize $x_0$ to be the zero matrix---which guarantees that $\rk(x_m)\le m$.
    We find that this algorithm could be efficiently implemented on GPU.


    \paragraph{Hardware.}
    We conducted all tests on a personal computer with 8 Cores i7-9700K 3.60GHz CPU, 64 GB of memory, and NVIDIA GEFORCE RTX 2080 SUPER with 8 GB of GPU memory.

    \paragraph{Computational details and notation.}
    Comprehensive comparisons among the methods introduced in \cref{sec:numerical tests spca} are detailed in \cref{tab:full_results}.
     We use ``Obj'' to denote the objective value of a solution found by a certain algorithm, ``Time'' to denote the runtime of an algorithm.
     Note that we run \cref{alg:multi_ra} for $n = 3000$ times, and report the largest objective value among those feasible solutions found in the column ``Obj'' belonging to ``\cref{alg:multi_ra}''. 
     For reproducibility, we set the random seed to 42.
    In the table, $c_0$ stands for $\textup{SSR} / \sqrt{k}$, measuring how far $\textup{SSR}$ is from $\sqrt{k}$.
    The column ``Total Time'' stands for the runtime of CGAL + \cref{alg:multi_ra}.
    We highlight the objective values that are largest among all algorithms for each instance.


    \begin{landscape}            % rotate this page
  \begin{table}[p]
    \caption{Complete numerical results for all 41 instances. Objective values and runtimes for each algorithm are reported. In the columns belonging to ``CGAL'', objective values for \ref{prob SDP SPCA} are reported, and $c_0$ stands for $\textup{SSR} / \sqrt{k}$. In the columns belonging to ``Algorithm~\ref{alg:multi_ra}'', ``Time'' stands for the runtime of \cref{alg:multi_ra} only, while ``Total Time'' stands for the runtime of CGAL + \cref{alg:multi_ra}.}
    \label{tab:full_results}
    \small               % compact font; tweak if needed
    \centering
    \adjustbox{max width=1.3\textwidth}{%
      \input{table_results_compact}   
    }
  \end{table}
\end{landscape}
